Efficient Listwise Reranking with Compressed Document Representations

Reranking, the process of refining the output from a first-stage retriever, is often considered computationally expensive, especially when using Large Language Models (LLMs). A common approach to mitigate this cost involves utilizing smaller LLMs or controlling input length. Inspired by recent advances in document compression for retrieval-augmented generation (RAG), we introduce RRK, an efficient and effective listwise reranker compressing documents into multi-token fixed-size embedding representations. Our simple training via distillation shows that this combination of rich compressed representations and listwise reranking yields a highly efficient and effective system. In particular, our 8B-parameter model runs 3x-18x faster than smaller rerankers (0.6-4B parameters) while matching or outperforming them in effectiveness. The efficiency gains are even more striking on long-document benchmarks, where RRK widens its advantage further.

==> latex/changes.tex <==


\section{Main Content}
\subsection{Section 1}
Write your notes for the first section here. You can include equations, lists, and other formatting as needed. For example:

\begin{itemize}
    \item Point 1
    \item Point 2
    \item Point 3
\end{itemize}

You can also include equations:
\[
E = mc^2
\]

\subsection{Section 2}
Continue with more sections and subsections to organize your notes.

\section{Conclusion}
Summarize your notes, conclusions, or any final thoughts here.



==> sections/03_rrk.tex <==

We build on the offline soft-compression framework PISCO \cite{pisco} to train a compressed reranking model called \textbf{RRK}\footnote{RRK: compressed version of \textbf{R}e\textbf{R}an\textbf{K}er}. RRK consists of two components: (i) a LoRA-finetuned PISCO compressor that maps documents to compressed token representations, and (ii) a LoRA-finetuned decoder reranker that assigns relevance scores to candidate documents conditioned on a query.

Let $\mathcal{D}=\{d_i\}_{i=1}^{N}$ denote a document collection and $q$ a query. The compressor $
f_{\theta_c}: d_i \rightarrow \mathbf{c}_i$ maps each document to a sequence of compressed embeddings: 
$\mathbf{c}_i = (c_i^1,\ldots,c_i^l)$ where $l$ is the number of memory tokens. Given a query and a candidate set $D_k=\{d_1,\ldots,d_k\}$ retrieved by a first-stage retriever, the reranker $
g_{\theta_r}(q,\mathbf{c}_1,\ldots,\mathbf{c}_k)$
produces relevance scores $s_i = g_{\theta_r}(q,\mathbf{c}_i)$
used to rank the documents.


\paragraph{Document Compression:}  After training the model, each collection is compressed \textbf{offline} using the finetuned  compressor: for each document $d_i$, a set of memory tokens $(m_1, \ldots, m_l)$ is appended, forming $(d_i; m_1, \ldots, m_l)$, which is fed to the compressor. The final $l$ hidden states of these memory tokens represent the document embeddings $\mathbf{c_i} = (c_i^s)_{s=1 \ldots l}$. In our case, we use a fix length of $l=8$ memory tokens, representing a x16 compression factor during PISCO training for a max-length of 128 tokens. We will show that the PISCO compressor naturally scales with longer documents (up to 2048 in our experiments, see Section~\ref{sec:longdoc}).


\paragraph{Listwise LLM Reranker} Our approach adopts an input representation similar to the Jina teacher \cite{wang2025jinarerankerv3lateinteractionlistwise}. The input sequence comprises query tokens (\textbf{in its textual representation}), followed by document memory tokens (\textbf{in their compressed representation}), and then the query tokens once more\footnote{Repeating the query at both the beginning and end may compensate for the lack of bidirectional attention and enhances the results}. %We use [SEP] tokens to separate documents, as employed in the PISCO model for document separation. More formally, the input to the LLM decoder is: $X=(q, \mathbf{c_1}, [\text{SEP}], \mathbf{c_2}, ,[\text{SEP}], \mathbf{c_3}, [\text{SEP}], q)$.
For a query $q$ and candidate documents $\{d_1,\ldots,d_k\}$, the decoder input sequence is
\[
X =
(q ; \mathbf{c}_1 ; [\text{SEP}] ; \mathbf{c}_2 ; [\text{SEP}] ; \ldots ; \mathbf{c}_k ; [\text{SEP}]; q)
\]
Let $H = \text{Decoder}_{\theta_r}(X)$
denote the hidden states produced by the reranker. The query representation is extracted from the final token
$\mathbf{q} = H_{|X|}$
while the representation of document $d_i$ is taken from the hidden state $\mathbf{h}_i$ corresponding to the separator token following its compressed tokens. The ranking score is then computed by cosine similarity $s_i = \cos(\mathbf{q},\mathbf{h}_i).
$

We use the RankNet listwise loss \cite{burges2005learning,gangi-reddy-etal-2024-first,E2Rank} to train RRK models.
Let $\mathcal{P}$ be the set of preference pairs $(d_i,d_j)$ where $d_i$ is preferred to $d_j$, the RankNet loss is parametrized by a temperature $\tau$\footnote{we use $\tau=1/8$} is:
\[
\mathcal{L}(q,D_k)
=
 \sum_{(i,j)\in\mathcal{P}}
\ \log(1+ \exp({ \frac{s_i - s_j}{\tau}}) )
\]

It is important to stress that the compressor is trained \textit{jointly} with the reranker, ie by backpropagating the ranking loss through the scores $s_i = g_{\theta_r}(q,f_{\theta_c}(d_i))$. After training, the documents are compressed offline and the decoder can be applied during inference to sort document by their scores.

Importantly, compression enables to reduce the reranking complexity. Let $k$ is the number of documents to be reranked and $|q|$ denote the number of query tokens and $|d|$ the average document length. A standard LLM reranker processes sequences of length $|q| + k|d|$, leading to an attention complexity of $\mathcal{O}((|q| + k|d|)^2)$. Our model instead processes sequences of length $2|q| + k(l+1)$, where $l$ is the number of memory tokens. The resulting complexity becomes $\mathcal{O}((2|q| + k(l+1))^2)$. Since $l \ll |d|$ (e.g., $l=8$ vs.\ $|d|\approx 200$ on average for most BeIR collections), this substantially reduces the quadratic attention cost of the reranker.





% \section{Experimental Setup}
% %   why here !!!!
% Our experiments are designed to address three main questions. First, we evaluate whether RRK achieves competitive effectiveness compared to more computationally expensive LLM-based rerankers. This comparison also implicitly assesses the quality of the PISCO embeddings used in RRK. Second, we analyze the latency of the models, with particular attention to performance on long documents where compression plays a critical role. Finally, we compare RRK to PE-Rank and E2RANK, examining whether our hypothesis—that compression learned through soft LLM-based methods yields more fine-grained representations than retrieval-based embeddings—is supported in practice.


% very bad formulation of research Q; EXp
%First, our experiments assess whether RRK is effective compared to an inefficient LLM Rerankers. This comparison will implicitly test the quality of PISCO embedding. Secondly, the latency of models will be analyzed, and a special analysis will be made on long documents. Finally, comparison with PE-Rank


\section{Experimental Framework}
\label{sec:training}
\paragraph{Distillation and Teacher}
Training high-quality rerankers usually requires large labeled datasets and carefully selected negatives from multiple retrievers \cite{cao2024recentadvancestextembedding}, making comparisons difficult and reducing reproducibility. Instead, we adopt a simpler approach based on distillation from a state-of-the-art reranker. Our goal is to evaluate whether rerankers trained on compressed document representations remain effective while improving efficiency. To this end, we distill a teacher into several models trained on a small dataset, including a base LLM, a ModernBERT baseline, and RRK. This setup enables a fair comparison between compressed and textual representations while remaining simple and reproducible. %as it requires no manual annotations.


%Training a high quality reranker depends on many factors such as labeled data with relevant documents and carefully chosen negatives from multiple retrievers, \cite{cao2024recentadvancestextembedding}. All these choices make comparison hard and reproducibility challenging due to varied and massive training sets.
%But, a simpler and more reproducible solution is to rely on \textit{distillation} from existing rerankers. In fact, our goal is to assess \textit{whether it is possible to train rerankers from compressed representations} and to assess their speedup
%%see whether LLM-based rerankers could be made faster.
%To do so, we take a state-of-the-art reranker and distill it into several model on a small dataset to draw a comparison between a base LLM, a modernBERT baseline and RRK models. 


%While stronger training configurations could be developed, our focus is comparing compressed vs. textual representations, making this configuration suitable for a fair evaluation. Our results shows that this distillation approach delivers good results, while offering a very simple setting (no annotation is required for training, and any collection can be used).




In order to select our teacher,  we performed a set of evaluation using various first-stage and rerankers.
%(see Appendix~\ref{appendix:teacher}).  No!
Based on those results, %and aiming at building an efficient full RAG system, 
we choose the SPLADE-V3 \cite{lassance2024spladev3newbaselinessplade}, a fast model proven to be robust out-of-domain, and the jina reranker V3\footnote{jinaai/jina-reranker-v3}, a listwise reranker based on a Qwen 0.6B  backbone \cite{wang2025jinarerankerv3lateinteractionlistwise}, which performs as well as the Qwen3-4B reranker. \citet{qwen3embedding} shows that larger LLMs (8B) perform similarly in terms of effectiveness. 


%A simple yet popular approach in natural language processing (NLP) is \textit{distillation}, which is used to "distil" large language models into smaller ones. We propose using this distillation process to train our reranker, but note that the distillation direction is inverted: from a small model to a larger one. We select a reranker as teacher, apply it on a well known dataset (MS-MARCO) and use this as training data. 



\paragraph{Training Set:}For our training collection, we first use the traditional MS MARCO (passage) dataset \cite{msmarco}. 
The training collection, which consists of a set of queries  and an appropriate document collection (without the need for relevance judgments), is processed using the selected first-stage retriever and reranker. For each query, we identify the top 50 documents produced by the reranker used as teacher. For the query set, we utilize the  0.5 million training queries, pairing each query with 16 documents randomly selected from the top 50 documents provided by the retriever. 
 %Stronger training configurations could certainly be developed; however, our primary objective is to evaluate the relevance of using compressed representations compared to textual ones. Therefore, we believe that this configuration enables a fair comparison of the two approaches
To evaluate this choice and to boost the results, a second collection, provided by \citet{E2rank2}, is also employed. This collection, derived from BGE-M3 \cite{qwen3embedding}, comprises 150,000 queries, each associated with 16 documents scored by Qwen-32B used as zero-shot teacher reranker. %The reranker used to select the document is Qwen 32B model used as zero-shot reranker.
%We refer to \textbf{RRK-MS} as the model trained only on the MS MARCO collection, and to \textbf{RRK} as the model trained on both collections.


\paragraph{Qwen Backbone
:} We select a Qwen backbone since the Qwen family provides multiple rerankers (our teacher and baselines). We train a PISCO model using the Qwen-2.5 8B-instruct model. The training of this PISCO-Qwen model precisely follows the methodology outlined by \citet{pisco}.


\paragraph{Pointwise LLM Reranker (RRK PW)} We also present a pointwise approach as comparison. At reranking stage, the compressed documents embeddings $\mathbf{c}$ are loaded and fed to the Decoder (Qwen-2.5 8B) finetuned for reranking. The model’s decoder takes as input the query (\textbf{in its textual representation}) along with the \textbf{compressed representation} of the document $\mathbf{c}$, and generates a score. We train the model with a mean squared error (MSE) loss to reproduce the scores of a teacher reranker. Specifically, a linear layer maps the final-layer representation of the last token to a scalar score.


To train our RRK models, we conduct training over 2 epochs, as additional epochs did not yield significant improvements. The finetuning takes 48h using 1 A100 GPU with 16 document per query, a batch size of 2, a learning rate of $1 \times 10^{-4}$, and gradient accumulation of 16.  For the pointwise version we use 4 documents per query and a batch size of 8 (similar training time).
Regarding latency, all computations were performed on a single A100 GPU unless otherwise specified. Across all configurations, we used a Across all configurations, we used a batch size of 128, corresponding to over 90\% GPU memory utilization, except for the baseline models at input length 512, for which we increased the batch size to 256.
At inference, RRK requires access to the compressed representations, which accounts for less than 10\% of total reranking time. We store embeddings in a Hugging Face dataset and fetch document embeddings with the \texttt{select()} function.

==> tables/datasetlength.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{l|l|r|r}
\toprule
\textbf{Dataset}       & \textbf{Domain}         & \textbf{Avg. Query Length (words)} & \textbf{Avg. Document Length (words)} \\ 
\midrule
TREC-COVID             & Biomedical              & 10                                 & 160                                   \\ 
NFCorpus               & Biomedical              & 6                                  & 232                                   \\ 
NQ                     & Wikipedia          & 9                                  & 78                                   \\ 
HotpotQA               & Wikipedia          & 12                                 & 46                                   \\ 
FiQA-2018              & Finance                 & 19                                 & 132                                   \\ 
Touché-2020            & Misc.           & 53                                 & 292                                   \\ 
Quora                  & Quora              & 9                                  & 11                                    \\ 
DBPedia                & Wikipedia             & 8                                  & 50                                    \\ 
SCIDOCS                & Scientific              & 11                                 & 176                                   \\ 
FEVER                  & Wikipedia           & 14                                 & 85                                    \\ 
Climate-FEVER          & Wikipedia           & 18                                 & 85                                  \\ 
SciFact                & Scientific          & 15                                 & 213                                   \\ 
\midrule
TREC-News              & News                    & 11                                 & 634                                   \\ 
Robust04               & News                    & 12                                 & 466                                   \\ 
MsMarco Document       & Web                    & 12                                 & 1131                                   \\ 
\bottomrule
\end{tabular}
\caption{Overview of our datasets with average query and document lengths.}
\label{tab:datasets_length}
\end{table*}

==> tables/latency.tex <==
\begin{table*}[ht]
\small
\centering

\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
                       &   \multicolumn{3}{c|}{\textbf{\uline{Quora}}}  &  \multicolumn{3}{c}{\textbf{\uline{SciFact}}} \\
                       &\textbf{Avg. Len}  & \textbf{NDCG@10} & \textbf{Latency} &  
                        \textbf{Avg. Len}  & \textbf{NDCG@10} &\textbf{Latency}  \\
\toprule                
% \multicolumn{7}{l}{\textbf{Maximum Input Length: 512}} \\
% \midrule
% ModernBERT-Large    & 99 &85.9 & \textbf{1} & 512 &75.3& \textbf{1}  \\
% Mistral 7B (bs=128) &105 &86.4 & x41        & 512 &77.2 & x18  \\
% Long-RRK            &37  &86.8 & x18        & 54  &75.9 & x1.9  \\       
% \midrule
%\multicolumn{7}{l}{\textbf{Maximum Input Length: 1024}} \\
%\midrule
ModernBERT-Large    & 99  &85.9 & \textbf{1} & 868 &75.4& \textbf{1} \\
Mistral 7B (BS=64)  & 105 &86.4 & x41           & 852 &77.3& x30 \\
FT-RRK            & 29  &86.8 & x18           & 45  &76.7& x1.8 \\         
FT-RRK-16L            &29 &87.0  &x14 &              45 &74.7 & \textbf{x0.9} \\   
\bottomrule
\end{tabular}
}

\bigskip

\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
                       &   \multicolumn{3}{c|}{\textbf{\uline{TREC-NEWS}}}  &  \multicolumn{3}{c}{\textbf{\uline{Doc DL 19}}} \\
                       &\textbf{Avg. Len}  & \textbf{NDCG@10} & \textbf{Latency} &  
                        \textbf{Avg. Len}  & \textbf{NDCG@10} &\textbf{Latency}  \\
\toprule                
% \multicolumn{7}{l}{\textbf{Maximum Input Length: 512}} \\
% \midrule
% ModernBERT-Large    & 512 &50.5& 1     & 512 &69.7& 1 \\
% Mistral 7B          & 512 &51.6 & x2.7 & 512 &69.8 & x5.2 \\
% Long-RRK            & 37  &50.2 & \textbf{x0.48} & 30 &69.5 & \textbf{x0.44} \\   
% \midrule
%\multicolumn{7}{l}{\textbf{Maximum Input Length: 1024}} \\
%\midrule
ModernBERT-Large    & 1024 &51.5& 1 & 1024 &70.2& 1 \\
Mistral 7B (BS64)         & 1024 &51.2& x10 & 1024 &69.2& x9 \\
FT-RRK            & 22   &52.0& \textbf{x0.42} & 20 &70.1??68.5? & \textbf{x0.40} \\         
FT-RRK-16            & 22   & 49.3 &\textbf{x0.27} & 20 & 67.8& \textbf{x0.14}\\         
\bottomrule
\end{tabular}
}

\caption{Latency comparison across different datasets for the ModernBERT, Mistral (no compress) and Long-RRK. The \textbf{Avg.Len} column corresponds to the average document length computed at batch level. Batch size is 256 except for the Mistral model (OOM with 1024 input length). While for collections where documents are short (Quora),  Long-RRK is not able to challenge ModernBert, as soon as the batch average length reaches 1024 tokens, Long-RRK becomes twice faster. }
\label{tab:latency_comparison}
\end{table*}
\begin{table*}[ht]
\small
\centering

\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
                       &   \multicolumn{3}{c|}{\textbf{Quora}}  &  \multicolumn{3}{c|}{\textbf{SciFact}} &  \multicolumn{3}{c|}{\textbf{TREC-NEWS}} &  \multicolumn{3}{c}{\textbf{Doc DL 19}} \\
                       &\textbf{Avg. Len}  & \textbf{NDCG@10} & \textbf{Latency} &  
                        \textbf{Avg. Len}  & \textbf{NDCG@10} &\textbf{Latency}  &   
                        \textbf{Avg. Len}  &\textbf{NDCG@10} & \textbf{Latency}  & 
                        \textbf{Avg. Len}  &\textbf{NDCG@10} & \textbf{Latency}     \\
\toprule                
 \multicolumn{13}{c}{\textbf{Maximun Input Length: 512}} \\
 \midrule
%Naver-DeBERTa-v3-Large &   \\                       
ModernBERT-Large       & 99 &85.9 & \textbf{1} & 512 &75.3&\textbf{ 1}  & 512 &50.5&1  & 512&69.7& 1 \\
Mistral 7B     bs=128       &105 &86.4 & x41&512   &77.2 & x18  &512  &51.6 & x2.7  &512 &69.8 &x5.2\\
Long-RRK                  &37 &86.8 &x18& 54 &75.9& x1.9  &37 &50.2 &  \textbf{ x0.48} &30& 69.5  &  x.44\\
%Long-RRK &  \\
%PISCO 16L ???             & &           &   &   &   \\
\midrule
 \multicolumn{13}{c}{\textbf{Maximun Input Length: 1024}} \\
 \midrule
%Naver-DeBERTa-v3-Large &   \\                       
ModernBERT-Large       & 99 &85.9 &\textbf{ x1.0} & 868 &75.4&\textbf{ x1.1}   & 1024 &51.5&x1.1  & 1024&70.2& x1.1 \\
Mistral 7B    (BD=64)        & 105& 86.4& x41 &852 &77.3& x30.0 &1024 & 51.2&  x9.9 & 1024 &  69.2&x9.0\\
Long-RRK                  & 37 & 86.8 &x18& 54&75.9& 1.75  & 37& 52.0&   \textbf{ x0.42}&30 &  70.1  &  \textbf{x0.40}\\
%Long-RRK &  \\
%sPISCO 16L ???             & &           &   &   &   \\
\bottomrule
\end{tabular}
}

\caption{Latency comparison.  }
\label{tab:lantecy}
\end{table*}


% % To change the table size, act on the resizebox argument `0.8`.
% \begin{table*}[ht]
% \small
% \centering

% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc|ccc|ccc}
% \toprule
%                        &    \multicolumn{3}{c|}{\textbf{SciFact}}  &  \multicolumn{3}{c|}{\textbf{Quora}} &  \multicolumn{3}{c|}{\textbf{TREC-NEWS}} &  \multicolumn{3}{c}{\textbf{Doc DL 19}} \\
%                        &\textbf{Batch Length}  & \textbf{NDCG@10} & \textbf{Latency} &  
%                         \textbf{Length}  & \textbf{NDCG@10} &\textbf{Latency}  &   
%                         \textbf{Length}  &\textbf{NDCG@10} & \textbf{Latency}  & 
%                         \textbf{Length}  &\textbf{NDCG@10} & \textbf{Latency}     \\
% \toprule                
%  \multicolumn{13}{c|}{\textbf{Maximun Input Length: 512}} \\
%  \midrule
% %Naver-DeBERTa-v3-Large &   \\                       
% ModernBERT-Large       & 512 &75.3& 33s    & 99  &85.9&  01:30.86 & 512 &50.5&23  & 512&69.7& 18 \\
% Mistral 7B            & &&   & &86.4 & &  &51.6 &01:02.00  & &69.8 &03:11.75 \\
% Long-RRK                  &38  && 63   & &86.8 &25min&21 &50.2 &  11s & & 69.5  & 6s\\
% %Long-RRK &  \\
% %PISCO 16L ???             & &           &   &   &   \\
% \midrule
%  \multicolumn{13}{c|}{\textbf{Maximun Input Length: 1024}} \\
%  \midrule
% %Naver-DeBERTa-v3-Large &   \\                       
% ModernBERT-Large       & 868 &75.4& 36s    & 99 &85.9 & 01:30.86& 1024 &51.5&26  & 1024&70.2& 20 \\
% Mistral 7B            & &77.2&10:48 & & 86.4& & & 51.5& & & 69.2 &\\
% Long-RRK                  & 38 && 63   & & 86.8 &25min& 21& 52.0&    11s & &  70.1  & 6s\\
% %Long-RRK &  \\
% %sPISCO 16L ???             & &           &   &   &   \\
% \bottomrule
% \end{tabular}
% }

% \caption{Latency comparison.  }
% \label{tab:lantecy}
% \end{table*}

% To change the table size, act on the resizebox argument `0.8`.
% \begin{table*}[ht]
% \small
% \centering

% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc|ccc|ccc}
% \toprule
%                        &   \multicolumn{3}{c|}{\textbf{Quora}}  &  \multicolumn{3}{c|}{\textbf{SciFact}} &  \multicolumn{3}{c|}{\textbf{TREC-NEWS}} &  \multicolumn{3}{c}{\textbf{Doc DL 19}} \\
%                        &\textbf{Length}  & \textbf{NDCG@10} & \textbf{Latency} &  
%                         \textbf{Batch Length}  & \textbf{NDCG@10} &\textbf{Latency}  &   
%                         \textbf{Length}  &\textbf{NDCG@10} & \textbf{Latency}  & 
%                         \textbf{Length}  &\textbf{NDCG@10} & \textbf{Latency}     \\
% \toprule                
%  \multicolumn{13}{c}{\textbf{Maximun Input Length: 512}} \\
%  \midrule
% %Naver-DeBERTa-v3-Large &   \\                       
% ModernBERT-Large       & 99 &85.9 & 01:30.86 & 512 &75.3& 33s   & 512 &50.5&23  & 512&69.7& 18 \\
% Mistral 7B            &105 &86.4 & x41&(bs=128)   &77.2 &10:48 x18  &512  &51.6 &01:02.00 x2.7  &512 &69.8 &01:33 x5.2\\
% Long-RRK                  &21 &86.8 &x18& 38+16 && 63 x1.9  &21+16 &50.2 &  11s  x0.48 &14+16& 69.5  & 6s  x.44\\
% %Long-RRK &  \\
% %PISCO 16L ???             & &           &   &   &   \\
% \midrule
%  \multicolumn{13}{c}{\textbf{Maximun Input Length: 1024}} \\
%  \midrule
% %Naver-DeBERTa-v3-Large &   \\                       
% ModernBERT-Large       & 99 &85.9 & 01:30.86 & 868 &75.4& 36s   & 1024 &51.5&26  & 1024&70.2& 20 \\
% Mistral 7B            & 105& 86.4& x41 &(852 bs=64) &77.3&:18:16.61 x30.0 &1024 & 51.2& 4:17 x9.9 & 1024 &  69.2&3:12 x9.0\\
% Long-RRK                  & 21 & 86.8 &x18& 38+16 &75.9& 63  1.75  & 21+16& 52.0&    11s x0.42&14+16 &  70.1  & 6s  x0.40\\
% %Long-RRK &  \\
% %sPISCO 16L ???             & &           &   &   &   \\
% \bottomrule
% \end{tabular}
% }

% \caption{Latency comparison.  }
% \label{tab:lantecy}
% \end{table*}

















==> tables/pe.tex <==
\begin{table}[h]

\tiny
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
 \multirow{2}{*}{\textbf{Dataset}} &  \multirow{1}{*}{\textbf{BM25}} &   \multirow{2}{*}{\textbf{RRK}}  &\multirow{2}{*}{\textbf{FT-RRK}} &  \multirow{2}{*}{\textbf{PE-RANK}}\\ 
   &  (retriever)  & & \\
\midrule
\textbf{BeIR} & & & \\
% NFcorpus & 0.3375 & 0.3887 & 0.3639 \\
% DBPedia-entity & 0.3180 & 0.4284 & 0.4005 \\
% SciFact & 0.6789 & 0.7684 & 0.6938 \\
% Touché-2020-v2 & 0.4422 & 0.3187 & 0.3306 \\
% TREC-COVID & 0.5947 & 0.8492 & 0.7749 \\
% Avg & 0.4746 & 0.5507 & 0.5127 \\ \midrule
% \textbf{TREC} & & & \\
% TREC DL-19 & 0.5058 & 0.7406 & 0.7048 \\
% TREC DL-20 & 0.4796 & 0.7011 & 0.6354 \\ 
NFCorpus & 33.8 & 38.2&\textbf{38.9} & 36.4 \\
DBPedia-entity & 31.8 &42.3 &\textbf{42.8} & 40.1 \\
SciFact & 67.9 &75.0 &\textbf{76.8} & 69.4 \\
Touché-2020-v2 & 44.2 &30.7& 31.9 & 33.1 \\
TREC-COVID & 59.5 & 81.4 &\textbf{84.9} & 77.5 \\
\midrule
\textbf{Avg} & 47.5 & 53.52 &\textbf{55.1} & 51.3 \\ \midrule
\textbf{TREC} & & & & \\
TREC DL-19 & 50.6 &69.5 &\textbf{74.1} & 70.5 \\
TREC DL-20 & 48.0 &66.6 &\textbf{70.1} & 63.5 \\ 
\end{tabular}
}
\caption{Comparison between RRK and PE-RANK. Same setting as in \cite{liu2025leveraging}: reranking 100 documents from BM25.}
\label{table:pe}
\end{table}

% \begin{table}[h]
% \centering
% \begin{tabular}{lcc}
% \toprule
% \textbf{Dataset} & \textbf{Method} & \textbf{Score} \\ 
% \midrule
% \multirow{2}{*}{Example 1} & BM25 & 0.45 \\
%  & retriever &  \\ % Empty cell under "Score"
% Example 2 & BM25 & 0.50 \\
% Example 3 & Another method & 0.60 \\
% \bottomrule
% \end{tabular}
% \caption{Small example table with multirow.}
% \end{table}


==> tables/table-trecnews.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table}[ht]
\tiny
\centering

\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|cccc}
\toprule
  BeIR/TREC-NEWS                     &       \multicolumn{4}{c}{\textbf{Document Length Input}} \\
                       &   \textbf{256}  & \textbf{512} & \textbf{768} & \textbf{1024} \\
\midrule                       
Naver-DeBERTa-v3-Large & 46.0            & 50.9       & 48.6          & 46.0   \\                       
ModernBERT-Large       &  47.4             & 50.5        & 51.2      & 51.5    \\
Mistral 7B            & 49.5              & 51.6        &52.3         &51.5\\
RRK                  &   46.4   & 51.6   & 51.9       & 51.9\\
Long-RRK              &  47.7   &50.2    & 51.1    &52.0          \\
PISCO 16L           ??   &    \\
ModernBert-Large Doc ??    &   \\
\toprule
  BeIR/Robust04                     &       \multicolumn{4}{c}{\textbf{Document Length Input}} \\
                       &   \textbf{256}  & \textbf{512} & \textbf{768} & \textbf{1024} \\
\midrule                       
Naver-DeBERTa-v3-Large &               &        &           &    \\                       
ModernBERT-Large       &  59.2           & 60.6        & 60.1      & 59.0    \\
Mistral 7B            &  59.9             & 61.5        &60.9         &59.2\\
RRK                  &   60.1   & 60.8   & 60.7      & 60.4\\
Long-RRK               & 60.1    & 59.9   & 61.0    & 60.9\\
%PISCO 16L              &    (x0.5)       & 0.50   & (x1.5)    &  (x2) \\
\toprule
  MS-Marco Document DL-2019                     &       \multicolumn{4}{c}{\textbf{Document Length Input}} \\
                       &   \textbf{256}  & \textbf{512} & \textbf{768} & \textbf{1024} \\
\midrule                       
Naver-DeBERTa-v3-Large &             &       &           &   \\                       
ModernBERT-Large       &          &   69.7 &       & 70.2    \\
Mistral 7B            &               &    69.8     & 69.2        &\\
RRK                  &   64.7   & 66.2   & 65.8       & 66.1\\
Long-RRK             &   65.3    & 69.5   & 69.5     &  70.1\\
%PISCO 16L              &    (x0.5)       & 0.50   & (x1.5)    &  (x2) \\
\midrule
  MS-Marco Document DL-2020                     &       \multicolumn{4}{c}{\textbf{Document Length Input}} \\
                       &   \textbf{256}  & \textbf{512} & \textbf{768} & \textbf{1024} \\
\midrule                       
Naver-DeBERTa-v3-Large &            &        &            &   \\                       
ModernBERT-Large       &  63.6           & 65.7       & 65.9      &  66.7   \\
Mistral 7B            &   65.6            &   67.8     & 67.6        & 67.5\\
RRK                  &    64.7   & 66.2   & 65.8       & 66.1 \\
Long-RRK             &   65.3    & 68.4   & 68.0     &  68.0            \\
\end{tabular}
}

\caption{[PLACEHOLDER] Reranking "Long" documents. Increasing the document length can enhance rerankers effectiveness without affecting 
 the efficiency of RRK models.}
\label{tab:long}
\end{table}


==> tables/table0.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]

\centering


\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l cccccc  ccc cccc cccc  }
\toprule
%\multirow{2}{*}{\textbf{First Stage}}&  &\multicolumn{4}{c}{\textbf{off-the-shell}}   \\ 
%\cmidrule(lr){3-6}  \cmidrule(lr){7-10} %\cmidrule(lr){9-11} 
Retriever 
& \texttt{BM25}
& \texttt{SPLADE-v3}
& \texttt{Mix}
& \texttt{BGE}
& BM25 & BM25 & BM25
& SPLADE-v3 &MIXB & BGE

\\
        &&&&& +&+&+&+&+&+\\
Reranker&&&&& DeBERTa & mix &BGE & DeBERTa & mix &BGE \\
\midrule
\textbf{BeIR} &\\
\midrule    % bm     spl    m      b     b+d    b+m    b+b     s+d
Trec-covid & 0.59 & 0.75 & 0.76 & 0.75 & 0.82 & 0.81 & 0.73     & 0.85 & 0.87 & 0.79\\
SCIDOCS    & 0.15 & 0.16 & 0.23 & 0.22 & 0.19 & 0.19 & 0.17     & 0.19 & 0.20 & 0.18\\
NQ         & 0.31 & 0.59 & 0.56 & 0.55 & 0.54 & 0.53 & 0.53      & 0.66 & 0.64 & 0.50\\
SciFact    & 0.68 & 0.71 & 0.74 & 0.74 & 0.76 & 0.74 & 0.70     & 0.76 & 0.75 & 0.69\\
FIQA       & 0.24 & 0.37 & 0.45 & 0.44 & 0.40 & 0.37 & 0.34     & 0.45 & 0.44 & 0.39\\
QUORA      & 0.79 & 0.81 & 0.89 & 0.89 & 0.85 & 0.76 & 0.80     & 0.84 & 0.70 & 0.75\\
NFCorpus   & 0.34 & 0.36 & 0.38 & 0.37 & 0.38 & 0.39 & 0.33     & 0.38 & 0.40 & 0.31\\
HotpotQA   & 0.63 & 0.69 & 0.72 & 0.74 & 0.73 & 0.76 & 0.78     & 0.74 & 0.74 & 0.84\\
DPPedia    & 0.32 & 0.45 & 0.45 & 0.44 & 0.42 & 0.43 & 0.43     & 0.49 & 0.49 & 0.49\\
FEVER      & 0.65 & 0.80 & 0.86 & 0.84 & 0.80 & 0.78 & 0.87     & 0.78 & 0.81 & 0.92\\
Climate-FEVER & 0.17& 0.23&0.34&0.28&0.24&0.24&0.31&0.25&0.27& 0.37\\
Touché v2  & 0.29 &  0.29 & 0.23    &  0.23  & 0.34 & 0.35     & 0.31     & 0.31 & 0.24  &0.24 \\
\midrule
AVG &0.43& 0.52 & \textbf{0.55} &0.54&0.54& 0.54& 0.53 &\textbf{0.56}& \textbf{0.56}& 0.54 \\
%\midrule
%\textbf{LOTTE}  &  \\
% pooled search test& \\
% pooled forum test& \\ 
\bottomrule
\end{tabular}
}

\caption{Which reranker should you use? Rerankers may strongly depend on the choice of first-stage retriever. NDCG@10. Rerankers consider the top 50 documents and a maximun document length of 256.}
\label{tab:whichreranker}
\end{table*}

%dragon        0.73  0.16  0.53  0.68 0.36  0.87  0.34   0.66 0.42  0.76    0.31   0.21
%dragon+ deberta rr  0.86  0.19  0.65  0.76  0.47   0.85  0.38  0.73 0.46  0.83   0.31    0.25
%dragon +bge     rr   0.72 0.18 0.58   0.69 0.37 0.76  0.30  0.78 0.47 0.91 0.26  0.34


% repllama
%bm25+ rankllama  0.70  0.11 0.52  0.56  0.36 0.70 0.30 0.68 0.33 0.54 0.37
% repllama+rankllama



==> tables/table1.1.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]
\centering
\tiny
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l |c|cc|cc|cc|cc|cc }
\toprule
%\multirow{2}{*}{\textbf{Reranker}}&  &\multicolumn{4}{c}{\textbf{off-the-shell}}   & \multicolumn{4}{c}{\textbf{Trained}}    \\ 
%\cmidrule(lr){3-6}  \cmidrule(lr){7-10} %\cmidrule(lr){9-11} 
 &
\textbf{SPLADE-V3} %\textbf{Avg. Length}
&  \multicolumn{2}{c}{\textbf{Naver-DeBERTa}}
&  \multicolumn{2}{c}{\textbf{ModernBERT}}
&  \multicolumn{2}{c}{\textbf{Mistral 7B}}
& \multicolumn{2}{c}{\textbf{RRK}}
& \multicolumn{2}{c}{\textbf{RRK 16 Layers}}
%& \textbf{RR}
%& \textbf{RR 16Layers}
\\
&(retriever)& 256&512&256&512&256&512&256&512&256&512 \\
\midrule
\textbf{TREC} &\\
\midrule
DL 19 &72.3  & 77.6& 77.6 &76.3&76.3&\textbf{ 77.9}&\textbf{77.9}&77.1&77.1&77.1&77.1\\
DL 20 & 75.4 & 75.4&75.4 &76.7& 76.7&76.9&76.9&\textbf{77.0}&\textbf{77.0}&75.8&75.8\\
\midrule 
\textbf{BeIR} &\\
\midrule
TREC-COVID &74.8& 87.4&88.2&88.0& \textbf{89.0}    & 85.3& 85.6&86.4&86.2&85.9&86.5\\
NFCorpus   &35.7& 37.8&37.6&38.2& 38.1   & 37.9&    38.5 &38.0&\textbf{38.7}&38.3&38.9\\
NQ         &58.6&65.7 &65.7&65.9&66.0    &67.1 &\textbf{67.2}  &66.5&66.8    &65.1&65.2 \\
HotpotQA   &69.2&74.4 &74.5 &75.3&\textbf{75.4}     &74.1 &74.1  & 73.4 &73.4  & 71.4& 71.5\\
FIQA       &37.4&47.1 &47.8 &46.7&47.6     &47.0 &\textbf{48.2}  &46.7&47.1&45.1&46.1\\
Touché 2020-v2 &29.3  & 31.2&33.5 &32.9&\textbf{35.2}     &31.6 &31.6 &28.6&28.9&29.4&28.7 \\
Quora      & 81.4&84.3& 84.3&86.0&86.0    &86.4& 86.4  &\textbf{87.0}&\textbf{87.0}& \textbf{87.0}&\textbf{87.0}\\
DBPedia    &45.0&48.8 &48.8&50.1&50.1    &\textbf{50.5} &\textbf{50.5}  &49.4&49.4& 49.1&49.1\\
SCIDOCS    &15.8&19.3 &19.2&19.5&19.2     &\textbf{20.1} &19.2  &19.4&19.5&19.4&19.5 \\
FEVER      &79.6&83.5 &86.5 &85.76&\textbf{88.4}     &84.2 &86.9 & 83.4&84.2& 81.2&81.7 \\
Climate-FEVER &23.3 & 25.0 &27.4  &   23.2&25.3   &23.9 &2\textbf{7.5} &25.9&25.9& 25.8&25.9\\
SciFact    &71.0&76.2 &75.8&75.3&75.4    &75.4 &\textbf{77.3}  &75.2&76.4& 75.4&74.5 \\
\midrule
\textbf{AVG} & 51.8  &\textbf{56.6} &\textbf{57.4} &\textbf{57.2} &\textbf{57.9} & \textbf{57.0}&\textbf{57.8} & \textbf{56.6} &\textbf{56.9} & \textbf{56.1}&\textbf{56.2} \\
%\midrule
%TREC-NEWS &41.6 & 0.46&50.9 & 47.4&50.5   &49.4 &\textbf{51.6} &46.6&51.2&47.4&50.1  \\
%Robust04  &47.6 & 60.1&\textbf{61.7}  & 59.2&60.6  &59.9 &61.5 &60.2&60.8  &57.5&58.5 \\
\midrule 
\textbf{LoTTe}  &  \\
\midrule
 pooled search  &53.3 &62.2&62.6 &62.1&62.5 &62.5&\textbf{62.9}& 62.4&62.6 & 61.4&61.1 \\
 pooled forum & 36.0& 45.8&46.4& 45.4&45.9 & 45.9& \textbf{46.4} &45.9&46.3 & 45.3&45.2\\ 
\bottomrule
\end{tabular}
}

\caption{
Evaluation ($nDCG@10 * 100$) of textual and compressed (RRK) rerankers . The top 50 of the SPLADE-v3 retrieved documents is used as input. 
%DebertaV3 (256) is used as reference for processing time. 
}
\label{tab:reranker}
\end{table*}


==> tables/table1.2.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]
\centering
%\small
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l |c|c|c|c|c|c||c }
\toprule
%\multirow{2}{*}{\textbf{Reranker}}&  &\multicolumn{4}{c}{\textbf{off-the-shell}}   & \multicolumn{4}{c}{\textbf{Trained}}    \\ 
%\cmidrule(lr){3-6}  \cmidrule(lr){7-10} %\cmidrule(lr){9-11} 
 &
\textbf{SPLADE-V3} %\textbf{Avg. Length}
&  \multicolumn{1}{c|}{\textbf{Naver-DeBERTa}}
&  \multicolumn{1}{c|}{\textbf{ModernBERT}}
&  \multicolumn{1}{c|}{\textbf{Mistral 7B}}
& \multicolumn{1}{c|}{\textbf{RRK}}
& \multicolumn{1}{c||}{\textbf{RRK-16L}}
& \multicolumn{1}{c}{\textbf{FT-RRK}}
\\
&(retriever)&(teacher) &&&&& delete? \\
\midrule
\textbf{TREC} &\\
\midrule
DL 19 &72.3  &    77.6 &76.3&\textbf{77.9}&77.1&76.5& 77.5\\
DL 20 & 75.4 &    75.4 &76.7&76.9&77.0&74.7& \textbf{77.6}\\
\midrule 
\textbf{BeIR} &\\
\midrule
TREC-COVID &74.8&88.2& \textbf{89.0}    &  85.6&86.2&86.5&87.1\\
NFCorpus   &35.7& 37.6&38.1   & 38.5 &\textbf{38.7}&38.9& 38.3\\
NQ         &58.6& 65.7&66.0    &67.2  &66.8    &65.3 &\textbf{67.5}\\
HotpotQA   &69.2&74.5 &\textbf{75.4}     &74.1  &73.4  & 71.7& 73.8\\
FIQA       &37.4&47.8 &47.6     &\textbf{48.2}  &47.1&45.9&47.7\\
Touché 2020-v2 &29.3  &33.5 &\textbf{35.2}     &31.6 &29.1&29.4 &31.1\\
Quora      & 81.4&84.3&86.0    &86.4  &\textbf{87.0}& 86.8&86.8\\
DBPedia    &45.0&48.8&50.1   &\textbf{50.5}  &49.4&49.4&49.8\\
SCIDOCS    &15.8&19.2&19.5  &19.2  &19.5&19.8 &\textbf{19.8}\\
FEVER      &79.6&86.5 &\textbf{88.4}     &86.9 &84.2& 81.7 &84.8\\
Climate-FEVER &23.3 &27.4  &  25.3   &27.5 &27.2&26.1&\textbf{28.2}\\
SciFact    &71.0    &75.8&75.4    &\textbf{77.3}  &76.4&74.7 &76.4\\
\midrule
\textbf{AVG} & 51.8   &\textbf{57.4} &\textbf{\underline{57.9}} &\textbf{57.8} &\textbf{57.1}&\textbf{56.4} &\textbf{57.6}\\
%\midrule
%TREC-NEWS &41.6 & 0.46&50.9 & 47.4&50.5   &49.4 &\textbf{51.6} &46.6&51.2&47.4&50.1  \\
%Robust04  &47.6 & 60.1&\textbf{61.7}  & 59.2&60.6  &59.9 &61.5 &60.2&60.8  &57.5&58.5 \\
\midrule 
\textbf{LoTTe}  &  \\
\midrule
 pooled search  &53.3 &62.2&62.5&\textbf{62.9}&62.6 &61.1 & 62.7\\
 pooled forum & 36.0& \textbf{46.4}&45.9 & \textbf{46.4}&46.3 & 45.2&\textbf{46.4}\\ 
 \midrule
 \textbf{AVG} & \textbf{44.7} & \textbf{54.3}&\textbf{54.2}&\textbf{\underline{54.7}}&\textbf{54.}5&\textbf{53.2}&\textbf{54.6}\\
 \midrule
 \textbf{"Long" Documents} & &&&&&&\\
 \midrule 
 TREC-NEWS & 41.8& 51.1 & 50.5 & \textbf{51.6 }& \textbf{51.6} &50.6 &52.0 \\ 
 Robust04 & 47.6 &\textbf{61.7} & 60.6 & 61.5 & 60.8&59.6 &61.0 \\
 DL 19 Doc  & 65.6 &69.8&\textbf{70.2} & 69.2 & 68.3& 69.8&70.1\\
 DL 20 Doc & 63.2 &68.2 & 65.7&\textbf{67.8}  &66.2&65.4 &68.7\\
  \midrule
 \textbf{AVG} &\ 54.6&\textbf{62.7}&\textbf{61.8}&\textbf{\underline{62.5}}&\textbf{61.7} & \textbf{61.1}&\textbf{62.9}\\
\bottomrule
\end{tabular}
}

\caption{
Evaluation ($nDCG@10 * 100$) of textual and compressed (RRK) rerankers . The top 50 of the SPLADE-v3 retrieved documents is used as input. Documents as truncated at 512 tokens. All models are able to reproduce (and even outperform) the teacher effectiveness. Our compressed reranker, RRK, is just 0.6 below (BeiR) or equal to its non compressed version. 
}
\label{tab:reranker}
\end{table*}


==> tables/tablelength.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]
\centering

\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l ccccc }
\toprule
\textbf{}
& \textbf{SPLADE-V3}
& \ \multicolumn{4}{c} {textbf{ModernBERT-large }}
 & & 64 & &128&256&512&768  \\
\midrule
TREC-COVID&0.75 &0.832
NFCorpus  & 0.36 &0.38 & 0.36 &0.38&0.37&&0.38&0.39\\
NQ        &0.59&0.66& 0.62& 0.65 &0.66& &0.67&0.67\\
HotpotQA&0.69  &0.74 &0.72&0.74&0.75&&0.74&0.75\\
FIQA & 0.37 &0.47&0.43 &0.47&0.45 &&0.47 &0.47\\
Touché 2020-v2 & 0.29  & 0.31 &0.31&0.32&0.31&&0.31&0.30\\
Quora &0.81 &0.84&0.83&0.86 &0.86&& 0.87&0.85\\
DBPedia&0.45&0.49&0.48&0.49 &0.50&& 0.51&0.51\\
SCIDOCS&0.16 &0.19&0.17&0.19 &0.20&& 0.20&0.20\\
FEVER &0.80&0.83&0.88&0.85 &0.86& &0.85 &0.85\\
Climate-FEVER  &0.23 &0.25&0.21&0.23& 0.25&& 0.26&0.25\\
SciFact  &0.71&0.76&0.63&0.76 &0.75&0.58& 0.76&0.77\\
AVG & \textbf{0.52}&\textbf{0.56} & \textbf{0.54}&\textbf{ 0.57}  &\textbf{ 0.57 } & & \textbf{0.57}& \textbf{0.57} \\
\midrule
\end{tabular}
}
\caption{Impact of Shortening Documents: While reducing document length speeds up processing, it significantly decreases effectiveness.}

\label{tab:length}
\end{table*}


==> tables/tablenocompr.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]
\centering

\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l ccccccccccc }
\toprule
%\multirow{2}{*}{\textbf{Reranker}}&  &\multicolumn{4}{c}{\textbf{off-the-shell}}   & \multicolumn{4}{c}{\textbf{Trained}}    \\ 
%\cmidrule(lr){3-6}  \cmidrule(lr){7-10} %\cmidrule(lr){9-11} 
\textbf{}
%& \textbf{Avg. Length}
& \textbf{SPLADE-V3}
&  \textbf{DeBERTa-v3}
&  \textbf{ModernBERT-base}
& \textbf{ModernBERT-large }
%& \textbf{Qwen 0.5?}
& \textbf{llama 1B} %  expQwen/30924
& \textbf{Mistral 7B} %  expnocompr old/10915 1p
& \textbf{LLama 8B}   % expQwen/30219
& \textbf{Qwen 7B} %  expQwen/30214
\\
 & (Retriever)  & (Teacher)  \\
%&&256\\
\midrule
%\textbf{TREC} &\\
%DL19 & \\
%DL20 &\\
\midrule
\textbf{BeIR} &\\
\midrule
TREC-COVID&0.75 &0.87&0.85  &0.88&0.86 &0.85&0.85 &0.85 \\
NFCorpus  & 0.36 &0.38 & 0.36 &0.38&0.37&0.38&0.38&0.39\\
NQ        &0.59&0.66& 0.62& 0.65 &0.66&0.67 &0.67&0.67\\
HotpotQA&0.69  &0.74 &0.72&0.74&0.75&0.74&0.74&0.75\\
FIQA & 0.37 &0.47&0.43 &0.47&0.45 &0.47&0.47 &0.47\\
Touché 2020-v2 & 0.29  & 0.31 &0.31&0.32&0.31&0.32&0.31&0.30\\
Quora &0.81 &0.84&0.83&0.86 &0.86&0.86& 0.87&0.85\\
DBPedia&0.45&0.49&0.48&0.49 &0.50&0.51& 0.51&0.51\\
SCIDOCS&0.16 &0.19&0.17&0.19 &0.20&0.20& 0.20&0.20\\
FEVER &0.80&0.83&0.88&0.85 &0.86&0.84 &0.85 &0.85\\
Climate-FEVER  &0.23 &0.25&0.21&0.23& 0.25&0.24& 0.26&0.25\\
SciFact  &0.71&0.76&0.63&0.76 &0.75&0.75& 0.76&0.77\\
\midrule
AVG & \textbf{0.52}&\textbf{0.56} & \textbf{0.54}&\textbf{ 0.57}  &\textbf{ 0.57 } & \textbf{ 0.57 }& \textbf{0.57}& \textbf{0.57} \\
\midrule
%Trec-news&11/634 &0.42 & \\
%Robust04 &15/466 &0.48 &\\
%\midrule 
%\textbf{LoTTe}  &  \\
%\midrule
% pooled search test& &0.53 &0.62\\
% pooled forum test& &0.36&0.46& \\ 
\bottomrule
\end{tabular}
}

\caption{
Evaluation (NDCG@10) of rerankers trained with\textbf{ no compression} using Naver-DeBERTa as teacher. The top 50 documents of the SPLADE-v3 retrieved documents is used as input. Maximum input length 256. 
}
\label{tab:rerankernocompr}
\end{table*}
% deberta 128 0.84   0.19  0.64  0.72  0.420.84 0.37 0.73 0.49   x x 0.30
